Hall A Annual Report 2014

Report of the experimental activities in Hall A at Thomas Jefferson National Accelerator Facility during 2013.

==> bcm_2014/bcm_2014_2_modi.tex <==
%\documentclass{article}
%\usepackage{epsfig}
%\usepackage{subfigure}
%\usepackage{amssymb}
%\usepackage{authblk}
%\usepackage{multicol}
%\usepackage{rotfloat}
%\usepackage[breaklinks=true,colorlinks=true,linkcolor=blue]{hyperref}

%\begin{document}

\subsection{Hall A BCM System Status }
\label{sec:BCM}

\begin{center}
$^1$R.~Pomatsalyuk, $^1$O.~Glamazdin, $^2$J.~Gomez,  $^2$R.~Michaels, $^2$L.~Myers \\
$^1$National Science Center Kharkov Institute of Physics and Technology, Kharkov 61108, Ukraine  \\
$^2$Thomas Jefferson National Accelerator Facility, Newport News, VA23606, USA  \\
\end{center}


The Hall A beam current monitor system consist of  two cavity monitors and a parametric current transformer (PCT, ''Unser''). It is designed to measure a continues electron beam ($\sim$500~MHz pulse rate). The schematic diagram of Hall A beam current monitor system is shown on Fig.~\ref{fig:pic1}. Two cavity monitors ''Upstream'' and ''Downstream'' are calibrated with respect to a Faraday Cup. The Unser is an absolute measuring device but it suffers of offset drifts equivalent to a couple of $\mu$A ~\cite{denard}. Its calibration can be checked 
 periodically by injecting a known current through a wire crossing the Unser toroid parallel to the beam direction.

% \begin{figure}[hbt]
%    \caption [BCM: The Hall A beam current monitor system.]{The Hall A beam current monitor system.}
%    \centering
%         \includegraphics[width=1.0\textwidth]{bcm_2014/bcm/figures/pic1}
%    \label{fig:pic1} 
% \end{figure}

\begin{figure}[!ht]
\begin{center}
\begin{minipage}[t]{0.68\textwidth}
\hrule height 0pt
\includegraphics[width=\textwidth]{bcm_2014/bcm/figures/pic1}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
\hrule height 0pt
\vskip -3mm
  \caption [BCM: The Hall A beam current monitor system.]{The Hall A beam current monitor system.}
   \label{fig:pic1} 
\end{minipage}
\end{center}
\end{figure}

In the past a two stage calibration procedure was used:

\begin{itemize}
   \item linearity test of the Hall A BCM cavities with respect to the {\bf Faraday Cup \#2}; 
   \item cross calibration of the Hall A Unser monitor with the {\bf Faraday Cup \#2}. 
\end{itemize}

The cavity monitor signal is split and sent through two parallel paths. One path leads to the old 1~MHz electronic box and another one is connected to a new digital receiver ~\cite{musson}. The AC output of 1~MHz electronic 
blocks is connected to a digital voltmeter (DVM) with EPICS readout. Three voltage-to-frequency converters (VtoF) per cavity provide a value of the instantaneous beam current to the DAQ system. Three VtoF converters are used 
to maximize the dynamic range.  

New digital receiver has FPGA logic on board and digital signal processing (flexibility to be customized for our goals).  It has also analog output from DAC (18~bits, compatible with old system) and digital interface (TTL, optical) for fast data transfer. The new digital receiver can be used also with beam position monitor (BPM). In 
that case it provides measure of an electron beam position.

More information about Hall A BCM/Unser can be found on the web-page.%
\footnote{http://hallaweb.jlab.org/equipment/BCM/}%

\subsubsection{Unser Status}
\label{sec:unserstatus}

As it was mentioned before, the Unser has offset drifts order of $\pm2~\mu$A rms at constant temperature and a slope of $\pm 5~\mu A / ^\circ$C that cannot be compensated in place. These numbers are not determined by the electronics but by the magnetic material used to build the sensor head (Vitrovac\textregistered6025) ~\cite{unser}. An example of the  Unser drifts taken during a 24~hours period at 5~sec sampling interval is shown on Fig.~\ref{fig:pic2}.

\begin{figure}[!ht]
\begin{center}
\begin{minipage}[t]{0.68\textwidth}
\hrule height 0pt
\includegraphics[width=\textwidth]{bcm_2014/bcm/figures/pic2}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
\hrule height 0pt
\vskip -3mm
   \caption [BCM: Scatter plot and histogram of Unser output offset.]{Scatter plot (top) and histogram (bottom) of Unser output offset measured during 24~hours (with 5~sec time interval).}
   \label{fig:pic2} 
\end{minipage}
\end{center}
\end{figure}


\begin{figure}[!ht]
\begin{center}
\begin{minipage}[t]{0.68\textwidth}
\hrule height 0pt
\includegraphics[width=\textwidth]{bcm_2014/bcm/figures/pic3}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
\hrule height 0pt
\vskip -3mm
   \caption [BCM: Unser wire calibration.]{Unser wire calibration with current source K224 for different ranges.}
   \label{fig:pic3} 
\end{minipage}
\end{center}
\end{figure}


% \begin{figure}[hbt]
%    \caption [BCM: Scatter plot and histogram of Unser output offset.]{Scatter plot (top) and histogram (bottom) of Unser output offset measured during 24~hours (with 5~sec time interval).}
%    \centering
%         \includegraphics[width=1.0\textwidth]{bcm_2014/bcm/figures/pic2}
%    \label{fig:pic2} 
% \end{figure}
% The Unser is equipped with a current calibration source type of  Keithley~K224. It is used to do wire calibration of Unser through EPICS network based soft-IOC. The results of Unser wire calibration for different ranges are shown on Fig.~\ref{fig:pic3}. Unser gain is very stable, it is  4~mV per 1~$\mu$A for both ranges, but offset is drifting from 80~mV to 85~mV. 

% \begin{figure}[hbt]
%    \caption [BCM: Unser wire calibration.]{Unser wire calibration with current source K224 for 
%              different   ranges.}
%    \centering
%         \includegraphics[width=1.0\textwidth]{bcm_2014/bcm/figures/pic3}
%    \label{fig:pic3} 
% \end{figure}

\subsubsection{New BCM receiver test }
\label{sec:receiver}

New digital BCM receiver was installed on November 2014 in the Hall A. The result of linearity test of both the new digital BCM receiver and the old 1~MHz BCM receivers with RF current source performed by J.~Musson and L.~Myers are shown on Fig.~\ref{fig:pic4}. %
\footnote{HALOG entry \#3306142 } % 
Both systems appear to be quite linear (the residuals are less than 1\% above 1~$\mu$A). The new receivers are linear up to 30~$\mu$A. The observed saturation at higher beam current (100~$\mu$A) was due to the chosen electronic gain. The gain can be changed to work at higher current. 

% \begin{figure}[hbt]
%    \caption [BCM: New and old BCM receiver calibration.]{The calibration of new digital BCM receiver (left) and old 1~MHz BCM receiver (right) with RF source.}
%    \centering
%         \includegraphics[angle=90, width=1.0\textwidth]{bcm_2014/bcm/figures/pic4}
%    \label{fig:pic4} 
% \end{figure}

\begin{figure}[!ht]
\begin{center}
\begin{minipage}[t]{0.68\textwidth}
\hrule height 0pt
\includegraphics[width=\textwidth]{bcm_2014/bcm/figures/pic4}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
\hrule height 0pt
\vskip -3mm
   \caption [BCM: New and old BCM receiver calibration.]{The calibration of new digital BCM receiver (left) and old 1~MHz BCM receiver (right) with RF source.}
   \label{fig:pic4} 
\end{minipage}
\end{center}
\end{figure}

\subsubsection{BCM/BPM Fast Readout for Hall A DAQs (in progress) }
\label{sec:project}

A fast readout of the beam current monitor and position monitor via the new digital receiver system is being develop. Here we summarize the requirement we are working to meet. Two modes of operation are considered,

{\bf Event mode} 

An event is a moment in time defined by a trigger from detectors. Events arrive randomly in time 
(see Fig.~\ref{fig:pic5}).

% \begin{figure}[hbt]
%    \caption [BCM: Event mode operation diagram.]{Event mode operation diagram.}
%    \centering
%         \includegraphics[width=0.9\textwidth]{bcm_2014/bcm/figures/pic5}
%    \label{fig:pic5} 
% \end{figure}

\begin{figure}[!ht]
\begin{center}
\begin{minipage}[t]{0.68\textwidth}
\hrule height 0pt
\includegraphics[width=\textwidth]{bcm_2014/bcm/figures/pic5}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
\hrule height 0pt
\vskip -3mm
   \caption [BCM: Event mode operation diagram.]{Event mode operation diagram.}
   \label{fig:pic5} 
\end{minipage}
\end{center}
\end{figure}

\begin{itemize}
   \item A snapshot of the BPM data, ideally with 5~$\mu$m resolution (RMS of distribution) and integrated over a time interval $\delta t$ which is smaller than {\it 1/fraster} or {\it 1/fmovement}. Here, {\it fraster} is the raster frequency (25~kHz) and {\it fmovement} is the (presumably low) frequency of other movements of the beam. So, ideally $\delta t \le 4~\mu sec$; if there is a phase lag of a few $\mu$sec between the raster and the data, because this could be calibrated out. 
   \item Other experiments could pick a longer integration time to achieve a higher accuracy per snapshot. It is recommended to let $\delta t$ be a control parameter which would be set infrequently, like maybe at the start of an experiment.
  \item Snapshots of the BCM data with the integration time few seconds.
  \item The beam charge integrated over the time of a ''run''. A run lasts 30 to 60 minutes, typically. The time of a run is provided by a logic gate from the Trigger Supervisor (TS Gate).
\end{itemize}	 

{\bf Parity mode}

The DAQ runs at a fixed frequency governed by the helicity control board. Helicity frequency is in range from 30~Hz up to 2~kHz (see Fig.~\ref{fig:pic6}).

\begin{itemize}
   \item BCM (or BPM) signals are integrated over the interval of the helicity (0.5~-~30~ms). In between   the helicity flips, there is blank off the integration for typically 100~$\mu$sec (MPS) to allow for the Pockels Cell at the polarized source to settle.
   \item The integration gate can be provided by the Hall A DAQ.
\end{itemize}

The consumers of the Event Mode are: 

\begin{itemize}
   \item HRS DAQ;
   \item SBS DAQ;
   \item Third arm DAQs (e.g. Bigbite). 
\end{itemize}

The consumers of the Parity Mode are: 

\begin{itemize}
   \item HAPPEX DAQ;
   \item Moller Polarimeter DAQ;
   \item Compton Polarimeter DAQ. 
\end{itemize}

There could be other DAQ systems that use these data. The BCM data readout unit is supposed to be a custom VME 
unit to receive serial data stream. The unit is under development. 

% \begin{figure}[hbt]
%    \caption [BCM: Parity mode operation diagram.]{Parity mode operation diagram.}
%    \centering
%         \includegraphics[width=0.9\textwidth]{bcm_2014/bcm/figures/pic6}
%    \label{fig:pic6} 
% \end{figure}

\begin{figure}[!ht]
\begin{center}
\begin{minipage}[t]{0.68\textwidth}
\hrule height 0pt
\includegraphics[width=\textwidth]{bcm_2014/bcm/figures/pic6}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
\hrule height 0pt
\vskip -3mm
   \caption [BCM: Parity mode operation diagram.]{Parity mode operation diagram.}
   \label{fig:pic6} 
\end{minipage}
\end{center}
\end{figure}


\begin{thebibliography}{3}

\bibitem{denard} J.C.~Denard {\it et al.}, Proceedings of the 2001 Particle Accelerator Conference,
 Chicago(2001), 2326.
\bibitem{musson} J.~Musson {\it et al.}, Proceeding of 2009 Particle Accelerator Conf.,Vancouver, 
BC, CA, May 2009.
\bibitem{unser} K.B.~Unser {\it et al.}, Proceedings of the third Beam Instrumentation Workshop, 1991, CEBAF, Newport News, VA.

\end{thebibliography}

%\end{document}









==> bcm_2014/bcm_2014_2_orig.tex <==
%\documentclass{article}
%\usepackage{epsfig}
%\usepackage{subfigure}
%\usepackage{amssymb}
%\usepackage{authblk}
%\usepackage{multicol}
%\usepackage{rotfloat}
%\usepackage[breaklinks=true,colorlinks=true,linkcolor=blue]{hyperref}

%\begin{document}

\subsection{Hall A BCM System Status }
\label{sec:BCM}

\begin{center}
$^1$R.~Pomatsalyuk, $^1$O.~Glamazdin, $^2$J.~Gomez,  $^2$R.~Michaels, $^2$L.~Myers \\
$^1$National Science Center Kharkov Institute of Physics and Technology, Kharkov 61108, Ukraine  \\
$^2$Thomas Jefferson National Accelerator Facility, Newport News, VA23606, USA  \\
\end{center}


The Hall A beam current monitor system consist of  two cavity monitors and a parametric current transformer (PCT, ''Unser''). It is designed to measure a continues electron beam ($\sim$500~MHz pulse rate). The schematic diagram of Hall A beam current monitor system is shown on Fig.~\ref{fig:pic1}. Two cavity monitors ''Upstream'' and ''Downstream'' are calibrated with respect to a Faraday Cup. The Unser is an absolute measuring device but it suffers of offset drifts equivalent to a couple of $\mu$A ~\cite{denard}. Its calibration can be checked 
 periodically by injecting a known current through a wire crossing the Unser toroid parallel to the beam direction.

\begin{figure}[!ht]
\begin{center}
\begin{minipage}[t]{0.68\textwidth}
\hrule height 0pt
\includegraphics[width=\textwidth]{bcm_2014/bcm/figures/pic1}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
\hrule height 0pt
\vskip -3mm
  \caption [BCM: The Hall A beam current monitor system.]{The Hall A beam current monitor system.}
   \label{fig:pic1} 
\end{minipage}
\end{center}
\end{figure}

% \begin{figure}[hbt]
%    \caption [BCM: The Hall A beam current monitor system.]{The Hall A beam current monitor system.}
%    \centering
%         \includegraphics[width=1.0\textwidth]{bcm_2014/bcm/figures/pic1}
%    \label{fig:pic1} 
% \end{figure}

In the past a two stage calibration procedure was used:

\begin{itemize}
   \item linearity test of the Hall A BCM cavities with respect to the {\bf Faraday Cup \#2}; 
   \item cross calibration of the Hall A Unser monitor with the {\bf Faraday Cup \#2}. 
\end{itemize}

The cavity monitor signal is split and sent through two parallel paths. One path leads to the old 1~MHz electronic box and another one is connected to a new digital receiver ~\cite{musson}. The AC output of 1~MHz electronic 
blocks is connected to a digital voltmeter (DVM) with EPICS readout. Three voltage-to-frequency converters (VtoF) per cavity provide a value of the instantaneous beam current to the DAQ system. Three VtoF converters are used 
to maximize the dynamic range.  

New digital receiver has FPGA logic on board and digital signal processing (flexibility to be customized for our goals).  It has also analog output from DAC (18~bits, compatible with old system) and digital interface (TTL, optical) for fast data transfer. The new digital receiver can be used also with beam position monitor (BPM). In 
that case it provides measure of an electron beam position.

More information about Hall A BCM/Unser can be found on the web-page.%
\footnote{http://hallaweb.jlab.org/equipment/BCM/}%

\subsubsection{Unser Status}
\label{sec:unserstatus}

As it was mentioned before, the Unser has offset drifts order of $\pm2~\mu$A rms at constant temperature and a slope of $\pm 5~\mu A / ^\circ$C that cannot be compensated in place. These numbers are not determined by the electronics but by the magnetic material used to build the sensor head (Vitrovac\textregistered6025) ~\cite{unser}. An example of the  Unser drifts taken during a 24~hours period at 5~sec sampling interval is shown on Fig.~\ref{fig:pic2}.


\begin{figure}[!ht]
\begin{center}
\begin{minipage}[t]{0.68\textwidth}
\hrule height 0pt
\includegraphics[width=\textwidth]{bcm_2014/bcm/figures/pic2}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
\hrule height 0pt
\vskip -3mm
   \caption [BCM: Scatter plot and histogram of Unser output offset.]{Scatter plot (top) and histogram (bottom) of Unser output offset measured during 24~hours (with 5~sec time interval).}
   \label{fig:pic2} 
\end{minipage}
\end{center}
\end{figure}


\begin{figure}[!ht]
\begin{center}
\begin{minipage}[t]{0.68\textwidth}
\hrule height 0pt
\includegraphics[width=\textwidth]{bcm_2014/bcm/figures/pic3}
\end{minipage}
\begin{minipage}[t]{0.3\textwidth}
\hrule height 0pt
\vskip -3mm
   \caption [BCM: Unser wire calibration.]{Unser wire calibration with current source K224 for different ranges.}
   \label{fig:pic3} 
\end{minipage}
\end{center}
\end{figure}


% \begin{figure}[hbt]
%    \caption [BCM: Scatter plot and histogram of Unser output offset.]{Scatter plot (top) and histogram (bottom) of Unser output offset measured during 24~hours (with 5~sec time interval).}
%    \centering
%         \includegraphics[width=1.0\textwidth]{bcm_2014/bcm/figures/pic2}
%    \label{fig:pic2} 
% \end{figure}
% The Unser is equipped with a current calibration source type of  Keithley~K224. It is used to do wire calibration of Unser through EPICS network based soft-IOC. The results of Unser wire calibration for different ranges are shown on Fig.~\ref{fig:pic3}. Unser gain is very stable, it is  4~mV per 1~$\mu$A for both ranges, but offset is drifting from 80~mV to 85~mV. 

% \begin{figure}[hbt]
%    \caption [BCM: Unser wire calibration.]{Unser wire calibration with current source K224 for 
%              different   ranges.}
%    \centering
%         \includegraphics[width=1.0\textwidth]{bcm_2014/bcm/figures/pic3}
%    \label{fig:pic3} 
% \end{figure}

\subsubsection{New BCM receiver test }
\label{sec:receiver}

New digital BCM receiver was installed on November 2014 in the Hall A. The result of linearity test of both the new digital BCM receiver and the old 1~MHz BCM receivers with RF current source performed by J.~Musson and L.~Myers are shown on Fig.~\ref{fig:pic4}. %
\footnote{HALOG entry \#3306142 } % 
Both systems appear to be quite linear (the residuals are less than 1\% above 1~$\mu$A). The new receivers are linear up to 30~$\mu$A. The observed saturation at higher beam current (100~$\mu$A) was due to the chosen electronic gain. The gain can be changed to work at higher current. 

\begin{figure}[hbt]
   \caption [BCM: New and old BCM receiver calibration.]{The calibration of new digital BCM receiver (left) and old 1~MHz BCM receiver (right) with RF source.}
   \centering
        \includegraphics[angle=90, width=1.0\textwidth]{bcm_2014/bcm/figures/pic4}
   \label{fig:pic4} 
\end{figure}

\subsubsection{BCM/BPM Fast Readout for Hall A DAQs (in progress) }
\label{sec:project}

A fast readout of the beam current monitor and position monitor via the new digital receiver system is being develop. Here we summarize the requirement we are working to meet. Two modes of operation are considered,

{\bf Event mode} 

An event is a moment in time defined by a trigger from detectors. Events arrive randomly in time 
(see Fig.~\ref{fig:pic5}).

\begin{figure}[hbt]
   \caption [BCM: Event mode operation diagram.]{Event mode operation diagram.}
   \centering
        \includegraphics[width=0.9\textwidth]{bcm_2014/bcm/figures/pic5}
   \label{fig:pic5} 
\end{figure}

\begin{itemize}
   \item A snapshot of the BPM data, ideally with 5~$\mu$m resolution (RMS of distribution) and integrated over a time interval $\delta t$ which is smaller than {\it 1/fraster} or {\it 1/fmovement}. Here, {\it fraster} is the raster frequency (25~kHz) and {\it fmovement} is the (presumably low) frequency of other movements of the beam. So, ideally $\delta t \le 4~\mu sec$; if there is a phase lag of a few $\mu$sec between the raster and the data, because this could be calibrated out. 
   \item Other experiments could pick a longer integration time to achieve a higher accuracy per snapshot. It is recommended to let $\delta t$ be a control parameter which would be set infrequently, like maybe at the start of an experiment.
  \item Snapshots of the BCM data with the integration time few seconds.
  \item The beam charge integrated over the time of a ''run''. A run lasts 30 to 60 minutes, typically. The time of a run is provided by a logic gate from the Trigger Supervisor (TS Gate).
\end{itemize}	 

{\bf Parity mode}

The DAQ runs at a fixed frequency governed by the helicity control board. Helicity frequency is in range from 30~Hz up to 2~kHz (see Fig.~\ref{fig:pic6}).

\begin{itemize}
   \item BCM (or BPM) signals are integrated over the interval of the helicity (0.5~-~30~ms). In between   the helicity flips, there is blank off the integration for typically 100~$\mu$sec (MPS) to allow for the Pockels Cell at the polarized source to settle.
   \item The integration gate can be provided by the Hall A DAQ.
\end{itemize}

The consumers of the Event Mode are: 

\begin{itemize}
   \item HRS DAQ;
   \item SBS DAQ;
   \item Third arm DAQs (e.g. Bigbite). 
\end{itemize}

The consumers of the Parity Mode are: 

\begin{itemize}
   \item HAPPEX DAQ;
   \item Moller Polarimeter DAQ;
   \item Compton Polarimeter DAQ. 
\end{itemize}

There could be other DAQ systems that use these data. The BCM data readout unit is supposed to be a custom VME 
unit to receive serial data stream. The unit is under development. 

\begin{figure}[hbt]
   \caption [BCM: Parity mode operation diagram.]{Parity mode operation diagram.}
   \centering
        \includegraphics[width=0.9\textwidth]{bcm_2014/bcm/figures/pic6}
   \label{fig:pic6} 
\end{figure}


\begin{thebibliography}{3}

\bibitem{denard} J.C.~Denard {\it et al.}, Proceedings of the 2001 Particle Accelerator Conference,
 Chicago(2001), 2326.
\bibitem{musson} J.~Musson {\it et al.}, Proceeding of 2009 Particle Accelerator Conf.,Vancouver, 
BC, CA, May 2009.
\bibitem{unser} K.B.~Unser {\it et al.}, Proceedings of the third Beam Instrumentation Workshop, 1991, CEBAF, Newport News, VA.

\end{thebibliography}

%\end{document}








